Insights on Training Neural Networks for QUBO Tasks

Current hardware limitations restrict the potential when solving quadratic unconstrained binary optimization (QUBO) problems via the quantum approximate optimization algorithm (QAOA) or quantum annealing (QA). Thus, we consider training neural networks in this context. We first discuss QUBO problems that originate from translated instances of the traveling salesman problem (TSP): Analyzing this representation via autoencoders shows that there is way more information included than necessary to solve the original TSP. Then we show that neural networks can be used to solve TSP instances from both QUBO input and autoencoders' hiddenstate representation. We finally generalize the approach and successfully train neural networks to solve arbitrary QUBO problems, sketching means to use neuromorphic hardware as a simulator or an additional co-processor for quantum computing.

==> txt/methodology.tex <==
\section{Methodology}
\label{sec:Concept}

The basic idea behind this paper was the observation that when creating a QUBO matrix for a given TSP problem, numerous fields are occupied with distances between cities to be visited. Then again, numerous fields are also assigned redundantly or without a value, due to the quadratic formulation of this problem. Therefore, our motivation is to check whether it is possible to compress the QUBO representation of a TSP instance using an autoencoder (AE). Building on this, the question arises whether the data representation compressed by the NN can serve as input for a convolutional neural network (CNN) in order to obtain the particular qubit configuration as output that solves the TSP problem. In this paper the TSP problem is chosen exemplary, any other NP-complete problem could also have been used.
